Easy Semantification of Bioassays

Biological data and knowledge bases increasingly rely on Semantic Web technologies and the use of knowledge graphs for data integration, retrieval and federated queries. We propose a solution for automatically semantifying biological assays. Our solution contrasts the problem of automated semantification as labeling versus clustering where the two methods are on opposite ends of the method complexity spectrum. Characteristically modeling our problem, we find the clustering solution significantly outperforms a deep neural network state-of-the-art labeling approach. This novel contribution is based on two factors: 1) a learning objective closely modeled after the data outperforms an alternative approach with sophisticated semantic modeling; 2) automatically semantifying biological assays achieves a high performance F1 of nearly 83%, which to our knowledge is the first reported standardized evaluation of the task offering a strong benchmark model.

==> Intro.tex <==
%catching starting
The process of automatic semantification of biological assays (bioassays) will speed up their digitalization and accessibility. That is possible considering the recent development in Natural Language Processing and Artificial Intelligence as explored in our recent works for this specific topic~\cite{anteghini2020representing,anteghini2020scibertbased}.\par
%paragraph on what is a bioassay
Biological assays are defined as standard biochemical test procedures used to determine the concentration or potency of a stimulus (physical, chemical, or biological) by its effect on living cells or tissues~\cite{hoskins1962uses,irwin1953statistical}. A bioassay should contain relevant information and basic procedures such as determine signal indicating biological activity, determine doses used, calculation methods etc. Also, the bioassay should always be qualified and validated \cite{little2019bioassaysection}.\par
%how to represent a bioassay with BAO
To organise and represent this amount of information, a BioAssay Ontology (BAO) is commonly adopted \cite{visser2011BAO,vempati2012formalizationBAO,abeyruwan2014BAO}, where the BAO describes chemical and biological screening assays and their related results to facilitate their categorization and data analysis \cite{visser2011BAO,abeyruwan2014BAO}.
On BioPortal (\href{https://bioportal.bioontology.org/}{https://bioportal.bioontology.org/}), the BAO on June 3 2021, showed a number of classes (the number of named and not anonymous classes) in the ontology of 7513 and a number of properties (the number of properties or slots in the ontology) of 227.
That amount of information requires a well structured organisation in order to improve the knowledge sharing and acquisition.\par

%ORKG
Semantified bioassays could be stored and visualized in Digital Libraries, such as the Open Research Knowledge Graph (ORKG)~\cite{jaradeh2019open}, in a structured and freely accessible way, allowing researchers to share their experiment and increase the amount of available knowledge for the scientific community.

%aim and cool intro conclusion
We present the first tool that allows scientists to easily upload bioassays and search for similar ones as well as compare these semantically structured bioassays on their key properties.

==> Methods.tex <==
\subsection{Database}
As reported in our previous works~\cite{anteghini2020representing,anteghini2020scibertbased}, we used a learning set which comprises an expert manually annotated collection of 983 semantified bioassays~\cite{schurer2011bioassay,vempati2012formalizationBAO}. Each bioassay has between 5 and 92 semantic statements at an average of 53. An example annotations is shown in Table~\ref{tab:statementseg} for a selected bioassay.\par
A semantic statement annotation can contain both numerical and categorical elements, thus complicating the creation of a model for automatic semantification. We then split the content of each bioassays in statements for the automatic semantification with our SciBERT and K-Means models and statements to use for a sequence labelling model. The two dataset are described in the following sections.




\begin{table}\label{tab:statementseg}
\small
\begin{tabular}{l} \\\toprule
\textsc{has temperature value} $\rightarrow$ \textsc{25 degree celsius} \\
\textsc{has incubation time value} $\rightarrow$ \textsc{20 minute} \\
\textsc{has participant} $\rightarrow$ \textsc{DMSO} \\
\textsc{has assay phase characteristic} $\rightarrow$ \textsc{homogeneous phase}\\
\bottomrule
\end{tabular}
\caption{\small{Four example semantic statement annotations (from 50 total) for PubChem Assay ID 360. Note, these statements are triples with subject ``bioassay.''}}
\end{table}


\subsubsection{Database for automatic semantification}

\begin{table}[]
    \centering
    \begin{tabular}{p{4cm}|p{4cm}|p{2.5cm}}\toprule
        Unique Statements LH & Unique Statements & Variability $\%$  \\\midrule
         top10 & 795 & 41.7\\
         top20 & 959 & 50.3\\
         top30 & 1492 & 78.3\\
         top40 & 1804 & 94.6\\
         top50 & 1866 & 97.9\\
         top60 & 1879 & 98.6\\
         top70 & 1896 & 99.5\\
         top80 (full dataset) & 1906 & 100.0\\\bottomrule
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}


\subsubsection{Database for sequence labelling}
\subsection{SciBERT based model for automatic semantificaiton}
\ma{We trained the SciBERT model \cite{beltagy2019scibert}  }


==> Relatedwork.tex <==
%paragraph on historical perspective on bioassay semantification
%historical perspective on bioassay semantification -- some questions that can be answered... when did the semantification initiative begin? how is it useful? what does it help with for bioinformatics researchers? how does it make life easier?

Normally, bioassays can be stored and accessed on PubChem~\cite{yanli2011pubchembio,wang2016pubchembioassay} which now contains more than 1.3M bioassays (22-06-2021). Only considering the period between 2015 and 2021, 389.835 new bioassays have been added to PubChem. \par
The amount of stored data is continuously increasing, however, to analyze a single bioassay is expert-specific and time-consuming. The process is not scalable for large-scale analyses, e.g. searching databases for related assays and comparisons or clustering similar entries. This requires the creation of new approaches to favour bioassays semantification, analysis, comparison and facilitate knowledge sharing.
The ultimate goal would be to obtain a fully-automated software that can easily transform a human-friendly bioassay annotation to a computer-friendly version.\par
Research toward fully automated parsing of research-related text \cite{attwood2010utopia,tkaczyk2015structuredmetadata} is growing but many scenarios are quite tolerant to error rates.
As a compromise hybrid approaches (manual/automatic) have been explored and showed promising results such as in Clark et. al 2014 \cite{clark2014semiauto} with the expectancy that `reducing the time required for scientists to annotate their assays, we can realistically advocate for semantic annotation to become a standard part of the publication procedure'. In addition, if the number of correctly annotated bioassay protocols grows, more training data will be available for a machine learning algorithm that will correspondingly improve its performances.\par

NLP is fast proceeding in developing ways to classify written documents in terms of classified tokens in a computer-friendly representation \cite{kang2013biomedtext,leaman2013diseasename,liu2011biomed,santorini1995penntagset}. Deep Learning (DL) approaches are often used in NLP and have been widely applied in the clinical domain \cite{wu2019dlnlpclinical}. Recurrent neural networks and word2vec embeddings are popular methods \cite{mikolov2013word2vec,wu2019dlnlpclinical} however Wu et al. 2019 already anticipated a significant increase in attention due to BERT \cite{devlin2019bert}.\par
The BERT model architecture \cite{devlin2019bert} and its derivatives, like SCIBERT \cite{beltagy2019scibert} and BIOBERT \cite{lee2019biobert}, is based on a multilayer bidirectional Transformer \cite{vaswani2017}. 
BERT is trained to predicting
randomly masked tokens and predicting whether
two sentences are consecutive. 
In our work, we explored and applied SCIBERT, which has been trained on scientific text, using a  WordPiece \cite{wu2016wordpiece} vocabulary on a scientific corpus (vocabulary of size 30k).
The scientific corpus consists of a random sample
of 1.14M papers (82\% form biomedical domain) from Semantic Scholar \cite{ammar2018,beltagy2019scibert}. 

==> Results.tex <==

\subsection{SciBERT based model for automatic semantificaiton performances}

\begin{table}[]
    \centering
    \begin{tabular}{p{3.5cm}|p{2cm}|p{2cm}|p{2cm}}
    \toprule
         Unique Statements LH & Precision & Recall & F1 score
         \\\midrule
         full dataset, 160RF & 0.33 & 0.94 & 0.49\\
         full dataset, 170RF & 0.37 & 0.94 & 0.54 \\
         full dataset, 180RF & 0.35 & 0.94 & 0.51 \\\bottomrule
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}


\begin{table}[]
    \centering
    \begin{tabular}{p{3.5cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}}
    \toprule
         Unique Statements LH & Precision & Recall & F1 score & test-time TPU & test-time CPU
         \\\midrule
         top 10, 180RF & 0.56 & 0.93 & 0.70 & 1m 2s & $>$ 20m \\
         top 20, 180RF & 0.50 & 0.93 & 0.64 & & \\
         top 30, 180RF &  0.49 & 0.94 & 0.65 & & \\
         top 40, 180RF & 0.35 &  0.96 & 0.51 & & \\
         top 50, 180RF & 0.39 & 0.94 & 0.55 & & \\
         top 60, 180RF & 0.40 & 0.95 & 0.56 & & \\ 
         top 70, 180RF & 0.37 &  0.95 & 0.53 & & \\          
         full dataset, 180RF & 0.35 & 0.94 & 0.51 \\\bottomrule
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{p{3.5cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}}
    \toprule
         Unique Statements LH & Precision & Recall & F1 score & test-time TPU & test-time CPU
         \\\midrule
         top 10, 170RF & 0.53 & 0.94 & 0.67 &  &  \\
         top 20, 170RF & 0.50 & 0.89 & 0.64 & & \\
         top 30, 170RF & 0.45 & 0.95 & 0.61 & & \\
         top 40, 170RF & 0.37 & 0.94 & 0.52 & & \\
         top 50, 170RF & 0.36 & 0.95 & 0.52 & & \\
         top 60, 170RF & 0.41 & 0.92 & 0.57 & & \\ 
         top 70, 170RF & 0.32 & 0.95 & 0.48 & & \\          
         full dataset, 170RF & 0.37 & 0.94 & 0.54 \\     
          \\\bottomrule
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

\subsection{Sequence Labelling Results}
\subsection{Sem-Bioassay}

\subsection{K-means clustering Results}

Labels frequency: 1
Cluster size: 500
Precision: 0.8196815325934431
Recall: 0.8457441231317468
F-score: 0.8325088984185609
